On the Verge of Solving Rocket League using Deep Reinforcement Learning and Sim-to-sim Transfer

Autonomously trained agents that are supposed to play video games reasonably well rely either on fast simulation speeds or heavy parallelization across thousands of machines running concurrently. This work explores a third way that is established in robotics, namely sim-to-real transfer, or if the game is considered a simulation itself, sim-to-sim transfer. In the case of Rocket League, we demonstrate that single behaviors of goalies and strikers can be successfully learned using Deep Reinforcement Learning in the simulation environment and transferred back to the original game. Although the implemented training simulation is to some extent inaccurate, the goalkeeping agent saves nearly 100% of its faced shots once transferred, while the striking agent scores in about 75% of cases. Therefore, the trained agent is robust enough and able to generalize to the target domain of Rocket League.

==> content/fundamentals.tex <==


\input{tables/physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Rocket League's Physical Game Mechanics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TODO:
    % Make bullet and psyonix impulses clear
    % Write empirical approach and show one figure
    % Write Suspension

The implementation of the Unity simulation originates from the so called \emph{RoboLeague} repository \cite{Roboleague2021}.
As this version of the simulation is by far incomplete and inaccurate, multiple fundamental aspects and concepts are implemented, which are essentially based on the physical specifications of Rocket League.
These comprise, for example, the velocity and acceleration of the ball and the car, as well as the concept of boosting.
Jumps, double jumps as well as dodge rolls are now possible and also collisions and interactions.
There is friction caused by the interaction of a car with the ground, but also friction caused by the air is taken into account.

However, some further adjustments are necessary.
Therefore, table \ref{tab:physics} provides an overview on all the material that was considered during implementing vital physical components, while highlighting distinct adjustments, which are different to the ones found in the references.
It has to be noted that most measures are provided in \emph{unreal units} (uu).
To convert them to Unity's scale, these have to be divided by $100$.

Some adjustments are based on empirical findings by comparing the outcome of distinct physical maneuvers inside both simulations.
A completely custom solution for realizing the car's suspension is implemented.
Both concepts are detailed next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Empirical Approach}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/dodge_alignment.pdf}
    \caption{Dogde Roll: Comparison with Rocket League's Ground Truth}
    \label{fig:dodge_alignment}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Suspension}
\label{sec:suspension}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Stichpunkte zur Suspension:

% Theoretisches Konstrukt entspricht dem aus dem zwischenbereicht.

% Bei 0 Gravitation ist das rad auf Höhe 0.

% das rad kann bis zu 3 uu über die Ruheposition eingedrückt werden, und bis zu 12 uu unter die ruheposition "ausgefahren" werden. Diese werte basieren auf schätzungen von rocket science

% Implementiert haben wir das so:

% 3 Trigger zonen an jeden rad umfassen den gesamten bereich, in dem sich das rad befinden kann (wenn es in der höhe verschoben wird)
% ein kreis oben, ein kreis unten und ein rechteck dazwischen

The physical suspension of cars consists of a compression area above the wheel's rest position, in which the suspension can be compressed (up to max. $3 \uu$), and an extension area below the wheel's rest position, in which the suspension is extended (up to max. $ 12 \uu$).
As long as the wheel is in the extension area, it does not apply any force to the car, but it is capable of registering the contact. The wheels not collide with the hitbox of the car.
Only when a wheel is pushed into the compression zone a force will be applied upwards along the suspension to the car, which is 0 in the rest position and becomes stronger while pushing the wheel into the compression zone.  
When the vehicle falls to the ground, the wheel is pushed into the compression zone of the suspension and the suspension applies a force to the vehicle that is opposite to the force of gravity, thus decelerating the vehicle.


==> content/fundamentals_old.tex <==
\newcommand{\uu}{\text {uu}}
\newcommand{\uus}{\frac{\text{uu}}{\text{s}}}
\newcommand{\uuss}{\frac{\text{uu}}{\text{s}^2}}
\newcommand{\rs}{\frac{\text{rad}}{\text{s}}}
\newcommand{\rss}{\frac{\text{rad}}{\text{s}^2}}


\input{tables/physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Rocket League's Physical Game Mechanics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TODO:
    % Bullet Impulse
    % Write Suspension

The implementation of the Unity simulation originates from the so called \emph{RoboLeague} repository \cite{Roboleague2021}.
As this version of the simulation is by far incomplete and inaccurate, multiple fundamental aspects and concepts are implemented, which are essentially based on the physical specifications of Rocket League.
These comprise, for example, the velocity and acceleration of the ball and the car, as well as the concept of boosting.
Jumps, double jumps as well as dodge rolls are now possible and also collisions and interactions.
There is friction caused by the interaction of a car with the ground, but also friction caused by the air is taken into account.

However, some further adjustments are necessary and described subsequently.
An additional impulse on the center of the ball is introduced which is called psyonix impulse and which allows a better prediction and control of collisions \cite{Mish2019}.
The simulation described in this paper uses a ball that is slightly differently scaled compared to Rocket League discussed in \cite{Mish2019}: the used radius of the ball is changed to $93.15\uu$, while using a radius of $91.25\uu$ in the same equation as shown by Mish.
The implementation in Unity contains the concepts of ball bouncing, ball-to-car interaction, and ground and wall stabilization, whereas a car-to-car interaction has not yet been fully implemented.

In the following, important aspects are discussed in detail.
The descriptions are based in particular on \cite{RLBotWiki2021}, \cite{Mish2019} and \cite{RocketScienceDodge2018}.
It has to be noted that most measures are provided in \emph{unreal units} (uu).
To convert them to Unity's scale, these have to be divided by $100$.
Some adjustments are based on empirical findings by comparing the outcome of distinct physical maneuvers inside both simulations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Velocity, Acceleration and Boost}
% @Jannik (Mittwoch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The maximum speed (i.e. the magnitude of the velocity) of a car in Rocket League is specified as $2300\uus$, while the maximum angular velocity is set to $5.6\rs$.
The car's acceleration on the ground is influenced by the throttle input.
If the sign of the car's forward velocity aligns with the sign of the throttle input, the car will accelerate according to the curve, described in \cite{Mish2019}.
In case the signs are opposite, the car will slow down with a constant deceleration of $3500\uuss$.
If no throttle is applied, the car is decelerated at a constant rate of $525\uuss$.
Boost is a consumable resource in Rocket League.
A car can have a maximum of $100$ boost in its tank and can only use the boost as long as the tank is not empty.
Boost can be collected through small and large boost pads around the field, which refill a car's tank with $12$ or $100$ boost respectively.
The positions and respawn timer of the boost pads on the field can be retrieved from \cite{RLBotWiki2021}.
While using boost, the throttle is set to $1$ and an additional $991.666\uuss$ of acceleration is applied in the car's forward direction.
The boost in the tank is reduced by $0.27$ in each frame resulting in a full tank being emptied in approximately $3.09$s.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Jump, Double Jump and Dodge Roll}
% @Jannik
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% QUELLE: https://github.com/RLBot/RLBot/wiki/Jumping-Physics

The jump immediately changes the car's velocity in its upward direction by $292\uus$.
The car will accelerate constantly by $1460\uuss$ for a minimum of three frames and a maximum of $0.2$s after the initial jump, depending on whether the jump was held or not.
A further $1.25$s after the end of the acceleration of the first jump and if the car is still in the air, the car may perform either a second jump or a dodge roll, depending on its rotational inputs.
When not using rotational inputs, a second jump will add an additional velocity of $292\uus$ in the relative upward direction, otherwise a dodge roll will be executed.
Dodge rolls were empirically analyzed in \cite{RocketScienceDodge2018}.
They last $0.65$s.
After the first $0.15$s, the car's vertical momentum is canceled by decreasing the velocity in the global upward direction by $35\%$ in each frame, so that the car moves almost only horizontally.
A torque is added according to the rotational input during the jump to increase the car's angular velocity to the maximum of $5.6\rs$.
It has been empirically proven that during a dodge roll the angular velocity increases to about $7.3\rs$, although Rocket League specifies a value of $5.6\rs$.

At the beginning of a dodge roll, the car changes its velocity.
The change depends on the direction of the car's movement $d_m$ and the rotational inputs, which need to be aligned with the car's forward direction.
The aligned rotational inputs direction is denoted with $d_i$ while the angle between $d_m$ and $d_i$ is denoted with $\varphi$.
The added velocity $v_d$ consists of a forward/backward ratio and a side-ward ratio and can be calculated via:
\begin{align}
v_{d} &= \begin{cases} 
    d_{c,f} \cos{\varphi} \cdot v_{d, f} + d_{c,s}(1-\cos{\varphi}) \cdot v_{d, s} & \text{if}~ \cos{\varphi} \geq 0\\
    d_{c,f} \cos{\varphi} \cdot v_{d, b} + d_{c,s}(1-\cos{\varphi}) \cdot v_{d, s} & \text{if}~ \cos{\varphi} < 0
\end{cases}\end{align}
where $d_{c,f}$ denotes the car's horizontal forward direction and $d_{c,s}$ the car's horizontal side-ward direction with 
\begin{align}
     v_{d,f} &= 500 \uus\\
     v_{d,s} &= 500 \uus \cdot \biggl(1+0.9\cdot\frac{||v_{forward}||}{2300\uus} \biggr) \\
     v_{d,b} &= 533 \uus \cdot \biggl(1+1.5\cdot\frac{||v_{forward}||}{2300\uus} \biggr)
\end{align}
(see also \cite{RocketScienceDodge2018})

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Air Control}
% @Jannik (Mittwoch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the air, the acceleration of the throttle is reduced to $66.667\uuss$ in forward gear and $33.334\uuss$ in reverse gear. % SOURCE: https://github.com/RLBot/RLBot/wiki/Jumping-Physics
Boost can still be used in the air with the same acceleration as on the ground.
This allows the car to fly through the arena.
The car can rotate around three axes determined by its forward direction (roll), its upward direction (yaw) and its sideways direction (pitch) with different torque and damping constants $(t, c)$ \cite{Mish2019}:

\input{tables/torqueAndDamping}
% Mir fällt gerade auf, dass wir die Konstanten angepasst haben könnten

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Collisions and Interactions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Bullet and Psyonix Impulse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Ball Bouncing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Ball-Car Interaction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ground and Wall Stabilization}
% @Jannik (Mittwoch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Stabilization forces are critical for the fast game-play of rocket league.
They are applied whenever the car touches the arena with a genuine subset of its wheels while using throttle.
If no wheel is touching the surface, only a torque is applied such that the car is rotating on its wheels.
If one to three wheels are in contact with the surface, an additional downward force of $325\uuss$ is pushing the car's center of mass to the ground. 
Sticky forces are applied to the car's center of mass, pushing it to its relative downward direction, while driving on the walls as mentioned in \cite{RLBotWiki2021}. To achieve Rocket-League-like behavior, the sticky forces are applied as acceleration of $500\uuss$ if the car is on non-ground arena surfaces, while the it has surface contact with at least two wheels. % Diese Kräfte sind zwar in der Quelle beschrieben, wir haben sie aber abweichend implementiert. Falls das Wandverhalten in 'future work' landet, dann sollte man den letzten Punkt evtl. dort mit aufgreifen.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Friction and Drifting}
% @Leon @Sebastian (Mittwoch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% GDC Talk https://www.gdcvault.com/play/1024972/It-IS-Rocket-Science-The
% Cite Cone2018
The key aspects regarding friction and drifting are described in \cite{Cone2018}.
For the behavior of a car, the lateral friction and the drag are relevant, but they are only important as long as the car moves on a surface.
The steering behavior of a car is mainly affected by lateral friction.
This Unity implementation uses a drag of $-525\uuss$, which is reduced by more than half when the car is on the roof.


% 2 verschiedene Arten: seitliche Reibung (lateral friction) und Bodenreibung (drag)

% beide nur relevant, wenn sich das Auto auf einer Oberfläche befindet

% Lenkverhalten vor allem durch die seitliche Reibung beeinflusst

% wird laut Quelle berechnet aus: Verhältnis von seitlicher undvorwärts-Geschwindigkeit, Koeffizient für die aktuell befahrene Oberfläche & physikalischer constraint

% Verhältnis von seitlicher und vorwärts-Geschwindigkeit wird in Funktion eingesetzt die definiert wird als f(x) in [0.2, 1] mit f(0) = 1, f(1) = 0.2

% genaue Funktion nicht bekannt, durch Versuche mit dem Physikabgleich-Tool sind wir auf folgenden Funktionsverlauf gekommen (siehe Bild)

% Implementierung bei uns ohne den Oberflächen-Koeffizienten, da wir diese nur am Boden betrachtet haben

% in RL: Oberflächen-Koeffizient: Oberflächen-Normale mit einer zweiten Funktion (Wertebereich + Funktion unbekannt)	physikalischer constraint: benötigter velocity change für sofortigen stillstand, folglich -1 * lateral wheel velocity

% drag: bei Reifen auf dem Boden: -525 uu/s^2, wenn auf dem Dach: geringerer Koeffizient

% in unity simulation berechnet als: coefficient / 4 * forwardSpeedSign * (1 - dragInputConstant)

% coefficient auf den Reifen: 5.25, auf dem Dach: 2.5

% dragInputConstant: maximum(Throttle-Input, boost-input) wobei boost-Input = 1 | 0


% Keine externen Quellen

% Implementierung des drifts über Anpassung der friction in CubeWheel

% Finden der Parameter über Physikabgleich

% Erkenntnis: drift und friction an der Wand ähnlich

% Anpassungen der friction:

% Impuls der lateral force für drift und Fahren an der Wand um Faktor 1/10 verkleinert

% Angriffspunkt der lateral force für drift und Fahren an der Wand weiter vorne

% mehr Drehung

% Angriffspunkt der Rotationskraft für drift und Fahren an der Wand weiter nach vorne

% mehr Drehung

% Keine autobreak/drag force für drift


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Suspension}
% @Frederik (Freitag)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Stichpunkte zur Suspension:

% Theoretisches Konstrukt entspricht dem aus dem zwischenbereicht.

% Bei 0 Gravitation ist das rad auf Höhe 0.

% das rad kann bis zu 3 uu über die Ruheposition eingedrückt werden, und bis zu 12 uu unter die ruheposition "ausgefahren" werden. Diese werte basieren auf schätzungen von rocket science

% Implementiert haben wir das so:

% 3 Trigger zonen an jeden rad umfassen den gesamten bereich, in dem sich das rad befinden kann (wenn es in der höhe verschoben wird)
% ein kreis oben, ein kreis unten und ein rechteck dazwischen



==> content/realted_work_backup.tex <==
% DotA 2
    % also high dimensional action space
    % also the issue of using mixed action spaces (continuous and discrete action spaces)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Sim-to-sim transfer on a popular multiplayer team video game touches on several different areas.
Therefore, in this section, we survey related work in the following fields:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-Agent Reinforcement Learning}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Multi-agent Reinforcement Learning (MARL) is a subfield in reinforcement learning research that addresses the issue of collaborative AI.
MARL methods have been successfully applied to several games in the past. One of the most popular applications is known as \textit{OpenAI Five} where a team of five neural networks defeated amateur human teams at Dota 2~\cite{DBLP:journals/corr/abs-1912-06680}.
Another milestone in MARL research has been reached by the successful application of MARL to the game Star Craft II which resulted in an AI which is able to compete on grandmaster level~\cite{DBLP:journals/nature/VinyalsBCMDCCPE19}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robocup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

RoboCup is an annual international competition~\cite{DBLP:conf/agents/KitanoAKNO97} that offers a publicly effective open challenge for the intersection of robotics and AI research and can be considered as a prime example for multi-agent scenarios.
RoboCup is mostly known for the robot soccer cup but also includes other challenges.
Reinforcement learning has been successfully applied to simulated robot soccer in the past~\cite{DBLP:journals/corr/HausknechtS15a} and has been found a powerful method for tackling robot soccer.
A recent overview that highlights significant trends and provides commentaries as well as insights for robot soccer is provided in \cite{AntonioniSRN21}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sim-to-real Transfer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Sim-to-real transfer is a well-established method for robot learning and is widely used
in combination with reinforcement learning.
In general, sim-to-real transfer allows the transition of a RL agent's behavior, which has been trained in simulations, to real-world environments.
Sim-to-real transfer has been predominantly applied to RL-based robotics~\cite{DBLP:conf/ssci/ZhaoQW20} where the robotic agent has been trained with state-of-the art RL techniques such as PPO~\cite{Schulman2017}, Soft Actor-Critic (SAC)~\cite{DBLP:conf/icml/HaarnojaZAL18}, Asynchronous Advantage Actor-Critic (A3C)~\cite{Mnih2016} and Importance Weighted Actor Learner Architecture (IMPALA)~\cite{Espeholt2018}. 
Popular applications for sim-to-real transfer in robotics have been autonomous racing~\cite{DBLP:conf/icra/BalajiMGGDKRSTT20}, Robot Soccer~\cite{DBLP:journals/corr/abs-1911-01529} navigation~\cite{DBLP:journals/corr/abs-1906-04452} and control tasks~\cite{DBLP:conf/icra/PedersenMC20}. 
To address the inability to exactly match the real-world environment, a challenge commonly known as sim-to-real gap, steps have been also been taken towards generalized sim-to-Real transfer for robot learning~\cite{DBLP:conf/cvpr/RaoHILIK20,DBLP:conf/icra/HoRXJKB21}. 
The translation of synthetic images to realistic ones at the pixel level is employed by a method called GraspGAN~\cite{DBLP:conf/icra/BousmalisIWBKKD18} which utilizes a generative adversarial network (GAN)~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14}. 
GANs are able to generate synthetic data with good generalization ability.
This property can be used for image synthesis to model the transformation between simulated and real images. GraspGAN provides a method called \textit{pixel-level domain adaptation}, which translates synthetic images to realistic ones at the pixel level.
The synthesized pseudo-real images correct the sim-to-real gap to some extent.
Overall, it has been found that the respective policies learned with simulations execute more successfully on real robots when GraspGAN is used~\cite{DBLP:conf/icra/BousmalisIWBKKD18}. 

% Domain randomization müsste noch rein



==> tables/alignment_backup.tex <==
\begin{table*}
\caption{The resulted mean, std and max error for each run physical maneuver scenario. The car's position is considered by the green shaded data points, while the blue ones are related to the ball's position.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r |
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r |
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r |
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r 
>{\columncolor[HTML]{F1FFF0}}r |
>{\columncolor[HTML]{EEEFFF}}r 
>{\columncolor[HTML]{EEEFFF}}r 
>{\columncolor[HTML]{EEEFFF}}r |
>{\columncolor[HTML]{EEEFFF}}r 
>{\columncolor[HTML]{EEEFFF}}r 
>{\columncolor[HTML]{EEEFFF}}r |}
\cline{2-19}
                                                         & \multicolumn{3}{c|}{\cellcolor[HTML]{F1FFF0}Acceleration}                                                    & \multicolumn{3}{c|}{\cellcolor[HTML]{F1FFF0}Air Control}                                                      & \multicolumn{3}{c|}{\cellcolor[HTML]{F1FFF0}Drift}                                                             & \multicolumn{3}{c|}{\cellcolor[HTML]{F1FFF0}Jump}                                                            & \multicolumn{3}{c|}{\cellcolor[HTML]{EEEFFF}Ball Bounce}                                                     & \multicolumn{3}{c|}{\cellcolor[HTML]{EEEFFF}Shot}                                                               \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{F4F4F4}Mean} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.69} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}3.72} & 1.67 & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}2.32} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}3.07} & 5.24  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}3.19}  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.84} & 4.87  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.07} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.22} & 1.37 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.01} & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.05} & 0.03 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}28.45} & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}23.79} & 28.31 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{F4F4F4}Std}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.48} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}3.05} & 1.92 & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}2.61} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}1.81} & 4.58  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}4.73}  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}1.04} & 6.8   & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.06} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.15} & 0.69 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.01} & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.03} & 0.02 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}25.2}  & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}25.01} & 22.49 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{F4F4F4}Max}  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}1.21} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}8.04} & 5.96 & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}8.4}  & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}8.12} & 12.97 & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}16.06} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}5.12} & 21.08 & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.24} & \multicolumn{1}{r|}{\cellcolor[HTML]{F1FFF0}0.41} & 2.02 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.02} & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}0.12} & 0.07 & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}58.16} & \multicolumn{1}{r|}{\cellcolor[HTML]{EEEFFF}59}    & 58.19 \\ \hline
\end{tabular}
}
\label{tab:align}
\end{table*}

==> tables/hyperparameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Hyperparameters ...}
\begin{tabular}{l|r}
\rowcolor[HTML]{EFEFEF} 
Hyperparameter        & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}Value} \\ \hline
Discount Factor        & 0.99                                              \\
\rowcolor[HTML]{EFEFEF} 
Lamda (GAE)            & 0.95                                              \\
Number of Workers      & 16                                                \\
\rowcolor[HTML]{EFEFEF} 
Worker Steps           & 512                                               \\
Batch Size             & 8192                                              \\
\rowcolor[HTML]{EFEFEF} 
Epochs                 & 3                                                 \\
Mini Batches           & 8                                                 \\
\rowcolor[HTML]{EFEFEF} 
Clip Range             & 0.2                                               \\
Max Gradient Norm      & 0.5                                               \\
\rowcolor[HTML]{EFEFEF} 
Value Loss Coefficient & 0.25                                              \\
Initial alpha          & 0.0003                                            \\
\rowcolor[HTML]{EFEFEF} 
Min alpha              & 0.000003                                          \\
Initial beta           & 0.0005                                            \\
\rowcolor[HTML]{EFEFEF} 
Min beta               & 0.00001                                           \\
Optimizer              & AdamW                                             \\
\rowcolor[HTML]{EFEFEF} 
Activations            & ReLU                                             
\end{tabular}
\label{tab:hyperparameters}
\end{table}

==> tables/torqueAndDamping.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}[h]{l|l|l}
 & torque & damping constant \\ \hline
 \rowcolor[HTML]{EFEFEF}
pitch & $t=12.15\rss$ & $c=-2.8$ \\
yaw & $t=8.92\rss$ & $c=-1.89$ \\
\rowcolor[HTML]{EFEFEF}
pitch & $t=36.08\rss$ & $c=-4.47$ \\
\end{tabular}
\label{tab:torqueAndDamping}
\ \\
